Passage Retrieval for Outside-Knowledge Visual Question Answering

In this work, we address multi-modal information needs that contain text questions and images by focusing on passage retrieval for outside-knowledge visual question answering. This task requires access to outside knowledge, which in our case we define to be a large unstructured passage collection. We first conduct sparse retrieval with BM25 and study expanding the question with object names and image captions. We verify that visual clues play an important role and captions tend to be more informative than object names in sparse retrieval. We then construct a dual-encoder dense retriever, with the query encoder being LXMERT, a multi-modal pre-trained transformer. We further show that dense retrieval significantly outperforms sparse retrieval that uses object expansion. Moreover, dense retrieval matches the performance of sparse retrieval that leverages human-generated captions.

==> 2_related_work.tex <==
%---------------------------------------------
\section{Related Work}
\label{sec:relatedwork}
%---------------------------------------------


==> tables/dense-results.tex <==
\setlength{\tabcolsep}{1pt}
\begin{table}[t]
\caption{Dense retrieval results. 
% Boldface denotes the best performance within each group and underscores denote the best results. $\blacktriangle i$ denotes that the gain with respect to method $i$ has statistically significance with $p < 0.05$ tested by the Student’s paired t-test.
Refer to Tab.~\ref{tab:sparse-results} for notations.
$\triangle i$ denotes the statistically significance is obtained with $0.05 < p < 0.1$. Note that BM25-Obj/Cap/All has access to the groundtruth object names and captions.}
\label{tab:dense-results}
\footnotesize
\vspace{-0.4cm}
\begin{tabular}{@{}l|l|ll|ll@{}}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{Methods}}      & \multicolumn{2}{c|}{Val}                             & \multicolumn{2}{c}{Test}                            \\ \cmidrule(l){3-6} 
\multicolumn{2}{c|}{}                              & MRR@5 & P@5 & MRR@5 & P@5 \\ \midrule
\multirow{4}{*}{\rotatebox{90}{Sparse}} & 1. BM25-Orig             & 0.2562                    & 0.1764                   & 0.2605                    & 0.1743                  \\
                        & 2. BM25-Obj (CombMAX)    & 0.3774$^{\blacktriangle 1}$                    & 0.2663$^{\blacktriangle 1}$                   & 0.3689$^{\blacktriangle 1}$                    & 0.2548$^{\blacktriangle 1}$                  \\
                        & 3. BM25-Cap (CombSUM)    & \textbf{0.4661}$^{\blacktriangle 1,2}$           & {\ul \textbf{0.3465}}$^{\blacktriangle 1,2,4,5}$     & {\ul \textbf{0.4638}}$^{\blacktriangle 1,2,4,5}$     & {\ul \textbf{0.3363}}$^{\blacktriangle 1,2,4,5}$   \\
                        & 4. BM25-All (CombMAX) & 0.4545$^{\blacktriangle 1,2}$                    & 0.3259$^{\blacktriangle 1,2}$                   & 0.4453$^{\blacktriangle 1,2}$                    & 0.3225$^{\blacktriangle 1,2,5}$                  \\ \midrule
\multirow{2}{*}{\rotatebox{90}{Dense}}  & 5. Dense-BERT            & 0.4555$^{\blacktriangle 1,2}$                    & 0.3155$^{\blacktriangle 1,2}$                   & 0.4325$^{\blacktriangle 1,2}$                    & 0.3058$^{\blacktriangle 1,2}$                  \\
                        & 6. Dense-LXMERT          & {\ul \textbf{0.4704}}$^{\blacktriangle 1,2\  \triangle5}$           & \textbf{0.3364}$^{\blacktriangle 1,2,5}$          & \textbf{0.4526}$^{\blacktriangle 1,2,5}$           & \textbf{0.3329}$^{\blacktriangle 1,2,5}$         \\ \bottomrule
\end{tabular}
\end{table}

==> tables/sparse-results.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\caption{Sparse retrieval results. Boldface denotes the best performance within each group and underscores denote the best overall results. $\blacktriangle i$ denotes that the gain with respect to the best method in group $i$ has statistically significance with $p < 0.05$ tested by the Student’s paired t-test.}
\label{tab:sparse-results}
\footnotesize
\vspace{-0.4cm}
\begin{tabular}{@{}l|c|ll|ll@{}}
\toprule
\multicolumn{2}{c|}{Methods}                     & \multicolumn{2}{c|}{Val}          & \multicolumn{2}{c}{Test}          \\ \midrule
\multicolumn{1}{c|}{Expansion}    & Fusion  & MRR@5           & P@5             & MRR@5           & P@5             \\ \midrule
1. BM25-Orig                    & N/A     & 0.2562          & 0.1764          & 0.2605          & 0.1743          \\ \midrule
\multirow{3}{*}{2. BM25-Obj}    & CombMAX & \textbf{0.3774}$^{\blacktriangle 1}$ & \textbf{0.2663}$^{\blacktriangle 1}$ & \textbf{0.3689}$^{\blacktriangle 1}$ & \textbf{0.2548}$^{\blacktriangle 1}$ \\
                                & CombSUM & 0.3486          & 0.2396          & 0.3401          & 0.2316          \\
                                & RRF     & 0.3367          & 0.2301          & 0.3295          & 0.2213          \\ \midrule
\multirow{3}{*}{3. BM25-Cap}    & CombMAX & 0.4545          & 0.3257          & 0.4458          & 0.3224 \\
                                & CombSUM & \underline{\textbf{0.4661}}$^{\blacktriangle 1,2,}$         & \underline{\textbf{0.3465}}$^{\blacktriangle 1,2,4}$          & \underline{\textbf{0.4638}}$^{\blacktriangle 1,2,4}$          & \underline{\textbf{0.3363}} $^{\blacktriangle 1,2,4}$         \\
                                & RRF     & 0.4654          & 0.3436          & 0.4582          & 0.3350          \\ \midrule
\multirow{3}{*}{4. BM25-All} & CombMAX & \textbf{0.4545}$^{\blacktriangle 1,2}$ & \textbf{0.3259}$^{\blacktriangle 1,2}$ & \textbf{0.4453}$^{\blacktriangle 1,2}$ & \textbf{0.3225}$^{\blacktriangle 1,2}$ \\
                                & CombSUM & 0.4471          & 0.3204          & 0.4412          & 0.3145          \\
                                & RRF     & 0.4309          & 0.3029          & 0.4264          & 0.2977          \\ \bottomrule
\end{tabular}
\end{table}
